BoschDreams-7V: Controllable Surround-View Video World Model for Long-Horizon Autonomous Driving

Closed-loop validation of autonomous driving requires surround-camera video streams that preserve 3D geometric coherence across overlapping views, remain visually stable over multi-minute rollouts, respond faithfully to counterfactual maneuvers, and run at real-time sensor rates. We present BoschDreams-7V, a controllable seven-camera world model that decouples physical state evolution from neural sensor synthesis. An explicit 3D simulator advances traffic dynamics and projects HDMap vectors and oriented 3D bounding boxes into each calibrated camera. This lets a 28-block causal Diffusion Transformer focus on photorealistic rendering over a sparse 7-edge (14-directed-edge) physical rig adjacency graph. A four-stage curriculum progresses from a bidirectional surround teacher and a block-causal student through few-step self-forcing distillation to Antiphon Forcing. This final stage combines a Layout-Aware Kernel Score (LAK) with role-decoupled writer and denoiser low-rank adapters and decoder vector-Jacobian memory backpropagation to resolve inter-role gradient conflict. Paired with exact in-place rotary position rebasing and compiled FP8 kernels, BoschDreams-7V delivers two operating points on a 600-scene surround benchmark. In the real-time 480p 1-step tier, it streams seven cameras synchronously at 10.85 FPS per camera (exceeding the 10 Hz camera clock) with 80.19 seven-view FVD, 7.02 m ego-trajectory ADE, and 119.53 late-window FVD (-68.0% vs. Stage III). In the high-fidelity 720p 4-step tier, it achieves 84.35 seven-view FVD (99.67 late-window FVD), 4.90 m ADE, and 380.50 cross-view LoFTR matches. As a stochastic flow-bridge fixer, it improves degraded 3D Gaussian Splatting renders by a mean of +1.26 dB PSNR (up to +2.12 dB) while reducing FID by 29.6% (up to 38.0%), FVD by 34.7% (up to 45.7%), and BEV feature distance (FBD) by 17.5% (up to 25.6%).

==> Makefile <==
# Build the Bosch technical-report template.
#   make           build report.pdf  (xelatex + bibtex, repeated until stable)
#   make template  build main.pdf    (the template example document)
#   make clean     remove auxiliary files       make distclean  ... and the PDFs
MAIN   ?= report
LATEX  ?= xelatex -interaction=nonstopmode -halt-on-error -file-line-error

.PHONY: all template clean distclean
all: $(MAIN).pdf

template: MAIN = main
template: main.pdf

$(MAIN).pdf: $(MAIN).tex boschreport.cls references.bib logo/boschlogo.pdf $(wildcard sections/*.tex) $(wildcard figures/*.pdf)
	$(LATEX) $(MAIN)
	-bibtex $(MAIN)
	$(LATEX) $(MAIN)
	$(LATEX) $(MAIN)
	@if grep -q "Rerun to get\|Label(s) may have changed" $(MAIN).log; then $(LATEX) $(MAIN); fi

main.pdf: main.tex boschreport.cls references.bib logo/boschlogo.pdf
	$(LATEX) main
	-bibtex main
	$(LATEX) main
	$(LATEX) main

clean:
	rm -f report.aux report.log report.out report.toc report.lof report.lot \
	      report.bbl report.blg report.brf report.synctex.gz report.xdv \
	      main.aux main.log main.out main.toc main.lof main.lot \
	      main.bbl main.blg main.brf main.synctex.gz main.xdv

distclean: clean
	rm -f report.pdf main.pdf

